An Exact Kernel Equivalence for Finite Classification Models

We explore the equivalence between neural networks and kernel methods by deriving the first exact representation of any finite-size parametric classification model trained with gradient descent as a kernel machine. We compare our exact representation to the well-known Neural Tangent Kernel (NTK) and discuss approximation error relative to the NTK and other non-exact path kernel formulations. We experimentally demonstrate that the kernel can be computed for realistic networks up to machine precision. We use this exact kernel to show that our theoretical contribution can provide useful insights into the predictions made by neural networks, particularly the way in which they generalize.

==> old_tex/old_figures.tex <==
\begin{tikzpicture}
% main step angles
\def\angA{72}
\def\angB{35}
\def\angC{15}
\def\angD{-20}

\def\nang{62}
\def\dang{45}
\def\sang{15}
\def\pang{30}

% \def\mang{29}
% \def\sang{39}
% \def\tang{50}
% \def\bang{60}
% \def\dang{34}

  \def\xs{1.0}
  \def\xa{4}
  \def\xe{1.0}
  \def\xd{0.75}
  \def\xn{0.5}
  \def\xi{1.4}
  % incoming edge
  \coordinate  (s1) at (0,0);
  \coordinate  (si1) at ($ (s1) + (\angA:1) $);
  \coordinate  (s2) at ($ (si1) + (\angA:\xs) $);
  \coordinate  (s3) at ($ (s2) + (\angB:\xa) $);
  \coordinate  (si3) at ($(s3) + (\angC:\xs) $);
  \coordinate  (s4) at ($(si3) + (\angC:\xs) $);

  %\node[fill=black,circle,inner sep=1.9] (s01) at (s1) {};
  \path (si1) -- (s2) node [midway, sloped] (elip) {\ldots};
  \path (s3) -- (si3) node [midway, sloped] (elip) {\ldots};
  \node[fill=black,circle,inner sep=1.9] (s01) at (s1) {};
  \node[fill=black,circle,inner sep=1.9] (s02) at (s2) {};
  \node[fill=black,circle,inner sep=1.9] (s03) at (s3) {};
  \node[fill=black,circle,inner sep=1.9] (s04) at (s4) {};
  %\node[fill=black,circle,inner sep=1.9] (s04) at (s4) {};

  \draw[black, line width=0.4mm, draw opacity=0.3] (s2) -- (s3);
\draw[black, line width=0.4mm, draw opacity=0.3] (s1) -- (si1);
\draw[black, line width=0.4mm, draw opacity=0.3] (si3) -- (s4);

\coordinate (p1) at (s2);%($ (s2)+(\ang:\xi) $);   % origin
\coordinate (p1n) at ($ (p1)+(\nang:\xe) $);       % ntk test

\coordinate (p1d) at ($ (p1)+(\angB+\sang:\xe) $); % dpk test

\coordinate (p1e) at ($ (p1)+(\angB+\sang:\xe) $); % epk test
\coordinate (p1t) at ($ (p1)+(\angD:\xe) $); % ntk train
\coordinate (p1b) at ($ (p1)+(\angB:\xe) $); % dpk epk train

\coordinate (p2) at  ($ (p1b)+(\angB:\xi) $);   % origin
\coordinate (p2n) at ($ (p2)+(\nang:\xe) $);       % ntk test
\coordinate (p2d) at ($ (p2)+(\angB+\sang:\xe) $); % dpk test
\coordinate (p2e) at ($ (p2)+(\angB+\pang:\xe) $); % epk test
\coordinate (p2t) at ($ (p2)+(\angD:\xe) $); % ntk train
\coordinate (p2b) at ($ (p2)+(\angB:\xe) $); % dpk epk train

\coordinate (p3) at  (s4); %($ (s4)+(\angB:\xi) $);   % origin
%   \draw[line width=10pt, ->, red] (0,0) -- (3,0);
%   \draw[line width=10pt, ->, blue] (0,0.5) -- (3,0.5);
  
%     \begin{scope}
%     \clip (-1,0) rectangle (3,1);
%     \draw[line width=10pt, ->] (0,0) -- (3,0);
%   \end{scope}
\coordinate (p3n) at ($ (p3)+(\nang:\xe) $);       % ntk test
\coordinate (p3d) at ($ (p3)+(\nang:\xe) $); % dpk test
\coordinate (p3e) at ($ (p3)+(\nang:\xe) $); % epk test
\coordinate (p3t) at ($ (p3)+(\angD:\xe) $); % ntk train
\coordinate (p3b) at ($ (p3)+(\angD:\xe) $); % dpk epk train

% \coordinate (p2) at ($ (p1a)+(\angB:0.6) $);
% \coordinate (p2a) at ($ (p2)+(\angB:\xe) $);
% \coordinate (p2b) at ($ (p2)+(\sang:\xe) $); 
% \coordinate (p3) at ($ (p2a)+(\angB:\xi) $);
% \coordinate (p3a) at ($ (p3)+(\angB:\xe) $);
% \coordinate (p3b) at ($ (p3)+(\tang:\xe) $);
% \coordinate (n0) at ($ (s1)+(\nang:\xn) $);
% \coordinate (n1) at ($ (p1)+(\nang:\xn) $);
% \coordinate (n2) at ($ (p2)+(\nang:\xn) $);
% \coordinate (n3) at ($ (p3)+(\nang:\xn) $);
% \coordinate (d0) at ($ (s1)+(\dang:\xd) $);
% \coordinate (d1) at ($ (p1)+(\dang:\xd) $);
% \coordinate (d2) at ($ (p2)+(\dang:\xd) $);
% \coordinate (d3) at ($ (p3)+(\dang:\xd) $);
    
% \draw[vector, ->, ntk] (s1) -- (n0) node[scale=1,above left=-3mm and 3mm, draw opacity=0.5] {$\vu{x}$};
% \draw[vector, ->, dpk] (s1) -- (d0) node[scale=1,above left=-3mm and 3mm, draw opacity=0.5] {$\vu{x}$};
\draw[vector, opacity=0.5, ->, ntk] (p1) -- (p1n) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%ntk test};

\draw[vector, opacity=0.5,  ->, dpk] (p1) -- (p1d) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%dpk test};

\begin{scope}
\clip (p1) -- (p1d) -- ($(p1d) + (0,1) $) -- ($ (p1) + (-1,1) $);
\draw[vector, ->, epk] (p1) -- (p1e) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%epk test};
\end{scope}
\draw[vector, ->, ntk] (p1) -- (p1t) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%ntk train};
\draw[vector, ->, epk] (p1) -- (p1b) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%(de)pk test};

\draw[vector, ->, ntk] (p2) -- (p2n) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%ntk test};
\draw[vector, ->, dpk] (p2) -- (p2d) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%dpk test};
\draw[vector, ->, epk] (p2) -- (p2e) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%epk test};
\draw[vector, ->, ntk] (p2) -- (p2t) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%ntk train};
\draw[vector, ->, epk] (p2) -- (p2b) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%(de)pk test};



\draw[vector, ->, ntk] (p3) -- (p3n) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%ntk test};
\draw[vector, ->, dpk] (p3) -- (p3d) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%dpk test};
\draw[vector, ->, epk] (p3) -- (p3e) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%epk test};
\draw[vector, ->, ntk] (p3) -- (p3t) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%ntk train};
\draw[vector, ->, epk] (p3) -- (p3b) node[scale=1,above left=-3mm and 3mm, draw opacity=0.2] {};%(de)pk test};

% \draw[vector, ->, epk] (p1) -- (p1b) node[scale=1,above left=-3mm and 3mm, draw opacity=0.5] {$\vu{x}$};
% \draw[vector, ->, epk] (p1) -- (p1a) node[scale=1,below left=1mm and 0mm, draw opacity=0.5] {$\vu{y}$};
% \draw[vector, ->, epk] (p2) -- (p2b) node[scale=1,above left=-3mm and 3mm, draw opacity=0.5] {$\vu{x}$};
% \draw[vector, ->, epk] (p2) -- (p2a) node[scale=1,below left=1mm and 0mm, draw opacity=0.5] {$\vu{y}$};
% \draw[vector, ->, epk] (p3) -- (p3b) node[scale=1,above left=-3mm and 3mm, draw opacity=0.5] {$\vu{x}$};
% \draw[vector, ->, epk] (p3) -- (p3a) node[scale=1,below left=1mm and 0mm, draw opacity=0.5] {$\vu{y}$};

\end{tikzpicture}

\begin{tikzpicture}
  \draw[line width=10pt, ->, red] (0,0) -- (3,0);
  \draw[line width=10pt, ->, blue] (0,0.5) -- (3,0.5);
  
    \begin{scope}
    \clip (-1,0) rectangle (3,1);
    \draw[line width=10pt, ->] (0,0) -- (3,0);
  \end{scope}
\end{tikzpicture}

\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {};
\node[draw,circle] (B) at (3,0) {};
\node[draw,circle] (C) at (0,3) {};
\draw[arr=green!30]   (A) -- (B);
\draw[arl=red!30]     (B.155) -- (C.291);
\draw[left=1.5mm, arr=blue!30]     (B.115) -- (C.339);
\end{tikzpicture}


\begin{tikzpicture}   
\draw [blue!80!white, very thick , ->, path fading=south,
  postaction={draw, green!80!white, path fading=north}]
  (0,0) .. controls +(0,-1) and +(0,1) .. (1,-2);
  \draw [blue!80!white, very thick , ->, path fading=south,
  postaction={draw, green!80!white, path fading=north}]
  (0,0) -- (1,-2);
    \draw [blue!80!white, very thick , ->, path fading=south,
  postaction={draw, green!80!white, path fading=north}]
  (0,0) -- (3,0);
   \draw [->, very thick] (0,0) -- (0,1);
    \draw [->, very thick, path fading=south] ([xshift=5pt, yshift=5pt]1,0) (1,0) -- (1,1);
\end{tikzpicture}

\begin{tikzpicture}
\draw[line width=10pt, ->, blue!80!black, path fading=south, top color=red!70!orange, bottom color=blue!70!orange!40!green] (0,1) -- (3,1);


%   \draw[line width=10pt, ->] (0,0) -- (3,0);
%   \shade[left color=red!70!orange, right color=yellow!70!orange] (0,0) rectangle (3,0.5);
%     \shade[left color=blue!70!orange, right color=yellow!70!orange] (0,0) rectangle (3,-0.5);
\end{tikzpicture}


% VECTOR breakdown in vectors
\begin{tikzpicture}
  \def\ul{0.52}
  \def\R{2.4}
  \def\ang{28}
  \coordinate (O) at (0,0);
  \coordinate (R) at (\ang:\R);
  \coordinate (X) at ({\R*cos(\ang)},0);
  \coordinate (Y) at (0,{\R*sin(\ang)});
  \draw[projcol,dashed] (X) -- (R);
  \draw[projcol,dashed] (Y) -- (R);
  \draw[vector] (O) -- (R) node[midway,left=5,above right=0] {$\vb{r}$};
  \draw[vector,<->,projcol]
    (X) node[scale=0.9,left=4,below=-1] {$x\vu{x}$} -- (O) --
    (Y) node[scale=0.9,below=4,left] {$y\vu{y}$};
  \draw[vector,<->,unitcol]
    (\ul,0) node[scale=0.9,left=2,below left=0] {$\vu{x}$} -- (O) --
    (0,\ul) node[scale=0.9,below=2,below left=0] {$\vu{y}$};
  %\draw pic[->,thick,"$\theta$",draw=black,angle radius=26,angle eccentricity=1.3]
  %  {angle = X--O--R};
\end{tikzpicture}


% VECTOR breakdown - all
\begin{tikzpicture}
  \def\ul{0.52}
  \def\R{2.6}
  \def\ang{28}
  \coordinate (O) at (0,0);
  \coordinate (R) at (\ang:\R);
  \coordinate (X) at ({\R*cos(\ang)},0);
  \coordinate (Y) at (0,{\R*sin(\ang)});
  \draw[projcol,dashed] (X) -- (R) node[scale=0.9,midway,right] {$y = r\sin\theta$};
  \draw[projcol,dashed] (Y) -- (R) node[scale=0.9,midway,above] {$x = r\cos\theta$};
  \draw[vector] (O) -- (R) node[midway,left=5,above right=0] {$\vb{r}$};
  \draw[vector,<->,projcol]
    (X) node[scale=1,left=4,below=-1] {$x\vu{x}$} -- (O) --
    (Y) node[scale=1,below=4,left] {$y\vu{y}$};
  \draw[vector,<->,unitcol]
    (\ul,0) node[scale=1,left=2,below left=0] {$\vu{x}$} -- (O) --
    (0,\ul) node[scale=1,below=2,below left=0] {$\vu{y}$};
  \draw pic[->,thick,"$\theta$",draw=black,angle radius=26,angle eccentricity=1.3]
    {angle = X--O--R};
\end{tikzpicture}


% VECTOR breakdown - all - velocity
\begin{tikzpicture}
  \def\ul{0.52}
  \def\R{2.6}
  \def\ang{28}
  \coordinate (O) at (0,0);
  \coordinate (R) at (\ang:\R);
  \coordinate (X) at ({\R*cos(\ang)},0);
  \coordinate (Y) at (0,{\R*sin(\ang)});
  \draw[projcol,dashed,veccol] (X) -- (R) node[scale=0.9,midway,right] {$v_y = v\sin\theta$};
  \draw[projcol,dashed,veccol] (Y) -- (R) node[scale=0.9,midway,above] {$v_x = v\cos\theta$};
  \draw[vector,vcol] (O) -- (R) node[midway,left=5,above right=0] {$\vb{v}$};
  \draw[vector,<->,vcol!90!black!60]
    (X) node[scale=1,left=4,below=-1] {$v_x\vu{x}$} -- (O) --
    (Y) node[scale=1,below=4,left] {$v_y\vu{y}$};
  \draw[vector,<->,unitcol]
    (\ul,0) node[scale=1,left=2,below left=0] {$\vu{x}$} -- (O) --
    (0,\ul) node[scale=1,below=2,below left=0] {$\vu{y}$};
  \draw pic[->,thick,"$\theta$",draw=black,angle radius=26,angle eccentricity=1.3]
    {angle = X--O--R};
\end{tikzpicture}


% VECTOR scaling
\begin{tikzpicture}
  \def\ul{0.52}
  \def\R{1.5}
  \def\ang{15}
  \draw[vector,myblue]
    (0,0) -- (\ang:\R) node[right=0] {$\vb{a}$};
  \draw[vector,mypurple,shift={(\ang-90:0.3)}]
    (\ang:\R) -- (0,0) node[above=0,left=0] {$-\vb{a}$};
  \draw[vector,myred,shift={(\ang+90:0.3)}]
    (0,0) -- (\ang:2*\R) node[right=0] {$2\vb{a}$};
\end{tikzpicture}


% VECTOR projection
\begin{tikzpicture}
  \def\ul{0.52}
  \def\R{3.3}
  \def\ang{25}
  \coordinate (O) at (0,0);
  \coordinate (R) at (\ang:\R);
  \coordinate (X) at ({\R*cos(\ang)},0);
  \draw[projcol,dashed] (R) -- (X);
  \draw[projcol,dashed] (-0.08*\R,0) -- (X) --++ (0.08*\R,0);
  \draw[vector,myblue] (O) -- (R) node[midway,left=5,above right=0] {$\vb{a}$};
  %\draw[vector,veccol!70]
  %  (O) -- (X) node[scale=0.8,left=4,below=-1] {$(\vb{r}\cdot\vu{x})\vu{x} = (r\cos\theta)\vu{x}$};
  %\node[myblue,scale=0.8,left=4,below=-1] at (X) {$\vb{a}\cdot\vu{x} = \abs{\vb{a}}\cos\theta$};
  \draw[myblue,<->]
    (O)++(0,-0.1*\R) --++ ({\R*cos(\ang)},0)
    node[scale=0.95,midway,fill=white,inner sep=1] {$\vb{a}\cdot\vu{x} = \abs{\vb{a}}\cos\theta$};
  \draw[vector,unitcol]
    (O) -- (\ul,0) node[scale=0.95,above=1,right=-1.5] {\contour{white}{$\vu{x}$}}; %,below left=0
  \draw pic[->,thick,"$\theta$",draw=black,angle radius=29,angle eccentricity=1.25]
    {angle = X--O--R};
\end{tikzpicture}


% VECTOR projection
\begin{tikzpicture}
  \def\ul{0.52}
  \def\R{3.1}
  \def\ang{26}
  \coordinate (O) at (0,0);
  \coordinate (R) at (\ang:\R);
  \coordinate (X) at ({\R*cos(\ang)},0);
  \draw[projcol,dashed] (R) -- (X);
  \draw[vector] (O) -- (R) node[midway,left=5,above right=0] {$\vb{r}$};
  \draw[vector,projcol]
    (O) -- (X) node[scale=0.8,left=4,below=-1] {$(\vb{r}\cdot\vu{x})\vu{x} = (r\cos\theta)\vu{x}$};
  \draw[vector,unitcol]
    (O) -- (\ul,0) node[scale=0.9,left=2,below left=0] {$\vu{x}$};
  \draw pic[->,thick,"$\theta$",draw=black,angle radius=26,angle eccentricity=1.3]
    {angle = X--O--R};
\end{tikzpicture}
